Smoothed Online Learning for Prediction in Piecewise Affine Systems

The problem of piecewise affine (PWA) regression and planning is of foundational importance to the study of online learning, control, and robotics, where it provides a theoretically and empirically tractable setting to study systems undergoing sharp changes in the dynamics. Unfortunately, due to the discontinuities that arise when crossing into different ``pieces,'' learning in general sequential settings is impossible and practical algorithms are forced to resort to heuristic approaches. This paper builds on the recently developed smoothed online learning framework and provides the first algorithms for prediction and simulation in PWA systems whose regret is polynomial in all relevant problem parameters under a weak smoothness assumption; moreover, our algorithms are efficient in the number of calls to an optimization oracle. We further apply our results to the problems of one-step prediction and multi-step simulation regret in piecewise affine dynamical systems, where the learner is tasked with simulating trajectories and regret is measured in terms of the Wasserstein distance between simulated and true data. Along the way, we develop several technical tools of more general interest.

==> body/noisy_alg.tex <==
%!TEX root = ../smoothonlineoptimistic.tex
\newpage
\newcommand{\labell}{\mathsf{label}}
\newcommand{\labeled}{\mathsf{prelab}}
\newcommand{\Fepoch}{\cF^{\mathrm{epoch}}}
\newcommand{\epsep}{\epsilon_{\mathrm{sep}}}
\newcommand{\Delsep}{\mathsf{\Delta}_{\mathrm{sep}}}
\newcommand{\N}{\mathbb{N}}
\section{Algorithms with Noise}

\subsection{Classification}
We consider 
\begin{itemize}
	\item Algorithm proceeds in epochs $s$ of length $\tau_s$
	\item For each epoch $s$, we have a lower bound $N_s$ on the size of a minimal ``good'' cluster (something in terms of MSE and separation). 
	\item We define the set of all clusters $C_s$ of size $\ge N_s$ at epoch $s$ as $\scrC_s$. 
	\item We define a ``probabilistic label'' as follows:
	\begin{align*}
	\forall C \in \scrC_s,  \labell(C) = \begin{cases} \labell(C_{s'}) & \text{ for any } C' \in \scrC_{s'} \text{ s.t. } \|\fhat_{C_{s,C}} - \fhat_{s',C'}\|_{\square} \le \epsep. \\
	\text{'something new'} & \text{otherwise} \\
	\end{cases}
	\end{align*} 
	We call the $C \in \scrC_s$ in the former case ``pre-labeled'', and call the set of such $C$'s $\labeled(\scrC_s)$. 
\end{itemize}

\begin{lemma} For all epochs $s$, there exist some $\pi_s$ such that, for all $s' \le s$, for all $C' \in \scrC_{s'}$
\begin{align*}
\{\#  z \in C': \pi_s(\labell(C')) \ne g_{\star}(z) \} \le \mathrm{ErrTerm} \approx \tilde{O}(\sqrt{\frac{1}{\Delsep|C'|}})
\end{align*}
\end{lemma}

\begin{lemma} Fix an epoch $s$. Given $s+1$,
\begin{align*}
\forall C \in \labeled(\scrC_{s+1}), \E[ | \Fepoch_s ]
\end{align*}
\end{lemma}

\subsection{Classification to Regression}
At each time $t$, fix an ERM, get $\fhat_{t,1},\dots,\fhat_{t,k}$. Then you devise a permutation $\pihat_t$ which ``aligns'' $\fhat_{t,i}$ ith labeled clusters. Then for new $x_t$, you predict $\ghat_t(x_t)$ from classifier. Then, you predice $\fhat_{t,\pihat_t(\ghat_t(x))}$. 

\begin{align*}
(\fhat_{t,\pihat_t(\ghat_t(x))} - \fst)^2 \le B^2 \I\{\pihat_t(\ghat_t(x)) \ne \gst(x) \} + (\fhat_{t,\pihat_t(\ghat)})
\end{align*}

\newpage

\section{More Formally}
\newcommand{\ErrTerm}{\mathrm{Err}}
\newcommand{\Mistake}{\mathrm{Mist}}
\begin{definition}[Error] We say a function $\ErrTerm(\cdot,\cdot): \N \times (0,1) \to \reals_{\ge 0}$ is an \emph{valid error term} if, with probability $1-\delta$, for all $s$ and all $C \in \scrC_s$,
\begin{align*}
\exists i \text{s.t. } \|\fst_i - \fhat_{C}\|_{2}^2 \le \ErrTerm(|C|,\delta). 
\end{align*}
\end{definition}

\begin{lemma} For a gamelength $T$ and minimal length $N_s$,  $\ErrTerm(N,\delta) \le \dots$ is a valid error term. 
\end{lemma}

\newcommand{\labst}{\mathsf{label}_{\star}}

\begin{lemma}\label{lem:true_assignment_noisy} Suppose that $\ErrTerm(N_s,\delta) < \Delsep^2/16$. Then, for every $s,s'$ and everu $C \in \scrC_{s}$, there exists
\begin{itemize}
\item Exactly one $i$ such that $\|\fst_i - \fhat_{C}\|_{2} < \Delsep/4$. We call this $\labst(C)$. 
\item at most one $C' \in \scrC_{s'}$ such that $\|\fhat_{C} - \fhat_{C'}\| < \Delsep/2$. 
\item If $\labst(C') = \labst(C)$, then $\|\fhat_{C} - \fhat_{C'}\| < \Delsep/2$.
\end{itemize} 

\end{lemma}

\begin{lemma}[Correctness of the Labeling Operator]
\end{lemma}
\begin{proof}
As a consequence of \Cref{lem:true_assignment_noisy}, for all clusters $C,C' \in \bigcup_{i=1}^s \scrC_s$, if $\labell(C) = \labell(C')$, then $\labst(C) = \labst(C')$. Set $\pi$ to be the correct permutation thats equivalence classes under $\labell$ to those under $\labst$.
\end{proof}

\begin{definition}[Mistake Term] We say a function $\Mistake(\cdot,\cdot): \N \times (0,1) \to \reals_{\ge 0}$ is an \emph{valid mistake term} if, with probability $1-\delta$, for all $s$ and all $C \in \scrC_s$,
\begin{align*}
\frac{1}{|C|}\sum_{(x,y) \in C} \I\{\gst(x) \ne \labst(C)\} = \frac{1}{|C|}\sum_{(x,y) \in C} \I\{\gst(x) \ne \pi_s \circ \labell(C)\} \le \Mistake(|C|,\delta).
\end{align*}
\end{definition}


==> body/noisy_reg.tex <==
%!TEX root = ../smooth_control_main.tex



\subsection{Setting}
We consider a sequential piecewiese affine regression setting. Consider a ground truth classification function $\gst: \R^d \to [K]$, as well as affine regression functions $(\bstA_k,\bstb_k) \in \R^{m \times d}\times \R^m$, for $k = 1,2,\dots,K$.

At each time step $t$, the adversary selects $\bz_t \in \R^d$, possibly adversarially. The learner then observes a smoothed iterate $\bx_t = \bz_t + \bw_t$, and covariate $\by_t$ given by
\begin{align*}
\by_t = \bstA_{k_t} \bx_t + \bstb_{k_t} + \be_t, \quad k_t := \gst(\bx_t)
\end{align*}
Importantly, $(\bx_t,\by_t)$ are revelead to the learner, but $k_t$ is not (neither are $\bz_t$, thought this is less essential). 
We consider two filtrations. First, $\filtz_t$ is the filtration generated by $\bz_1,\dots,\bz_t$ and $\bw_1,\dots,\bw_{t-1}$. Second $\filtx_t$ is the filtration generated by $\bz_1,\dots,\bz_t$ and $\bw_1,\dots,\bw_{t}$, and $\be_{1},\dots,\be_{t-1}$. Note that $\filtx_t \supset \filtz_t$, and that $(\bx_t)$ is $(\filtx_t)$ adapted. We furhter let $\barbx_t = (\bx_t,1)$, and $\Thetst_k = \begin{bmatrix} \bstA_k \mid \bstb_k\end{bmatrix}$. 
\begin{assumption} $\be_t \mid \filtx_t$ is $\sige^2$-subGaussian.
\end{assumption}
\begin{assumption} For all $t$, $\|\bz_t\| \vee \|\barbx_t\| \le B$.
\end{assumption}



\section{Analysis}



Fix a ground-truth classifer $\gst$, as well as an estimated classifer $\ghat \in \Gclass$. Given $(a,b) \in [K]^2$, introduce 
\begin{align*}
Z_{t;ab}(g) := \I\{g(\bx_t) = a, \gst(\bx_t) = b\}, \quad 
\Zbar_{t;ab}(g) := \Exp[Z_{t;ab}\mid \filtz_t]
\end{align*}
That is, $\Ztij$ is the indicator that a $\ghat$ assigned $\bx_t$  to cluster $b$ instead of its ground truth $a$, and $\barZtab$ is the expectation of this event given $\bz_t$, under the smooth noising $\bw_t$. Consider forward, let $\barbv \in \R^{d+1}$ denote vectors of the form $(\bv,b_0) = (v_1,\dots,v_d,v_0)$; the indexing designates $v_0$ as a distint, `affine entry'. We also denote $\barbx_t := (\bx_t, 1)$ in the same form


\subsection{A small-ball lemma.}


Our analysis describes on the regularity of the distribution $\bw$. Let $\Prw$ denote the distribution of $\bw$, and let $\Expw$ and $\Varw$ denote expectations and variances. Let $\disg$ denote the collection of sets of $\R^d$ of the form $\{\bx: g_1(\bx - \bmu) = a,g_2(\bx - \bmu) = b\}$, where $g_1 \ne g_2 \in \Gclass$, $\bmu \in \R^d$ and $a \ne b \in [K]$. 

\begin{definition}  Introduce the set-valued, $\filtz_t$-adapted random variable $\Wtab = \Wtab(g) := \{\bw \in \R^d: \ghat(\bz_t + \bw_t) = a, \gst(\bz_t + \bw_t) = b\}$.  For $\bdelta \in S^{d-1}$, define

\begin{align*}
\rho_t(g,\bdelta) &:= 
\frac{1 \wedge \Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]^2}{(1 +  \langle \bdelta, \bz_t \rangle^4 +  \Expw[\langle \bw,\bdelta \rangle^4 \mid \bw \in \Wtab])^2} \\
\zeta_t^2(g,\bdelta) &:= \frac{\Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]}{1\vee \left(\langle \bz_t, \bdelta\rangle^2 +   \Expw[\langle \bw, \bdelta \rangle ^2\mid \bw \in \Wtab]\right)},
\end{align*}
Define $\rho_t(g) := \inf_{\bdelta \in S^{d-1}} \rho_t(g,\bdelta)$ and define $\zeta(g) := \inf_{\bdelta \in S^{d-1}} \zeta_t(g,\bdelta)$
\end{definition}
\begin{restatable}{lemma}{lemsmallball}\label{lem:small_bal} There exist universal constants $c_0,c_1$ such that, for any $\barbv \in \cS^d$ with $\bv \ne 0 $,
\begin{align*}
\Pr\left[\langle \barbx_t, \barbv \rangle^2 \ge c_0 \zeta_t^2(\bdelta) \mid \filtz_t, \Ztij(g) = 1\right] \ge c_1 \rho_t(\bdelta).
\end{align*}
\end{restatable}
\begin{remark} The above is true independent of the functional form of $g$ and $\gst$.
\end{remark}
\begin{lemma}[Lower bound in terms of $\barZtab$]\label{lem:sigmarholowerbound}
	Suppose that $\inprod{\bw}{\bdelta}$ is $\sigma(\bdelta)$ smooth with respect the Lebesgue measure.  Then the following holds:
	\begin{equation}
		\Varw\left[\inprod{\bw}{\bdelta}| Z_{t;ab}\right] \geq \frac 12 \cdot \sigma(\bdelta)^2 \Zbar_{t;ab}^2
	\end{equation}
	In particular, it holds that
	\begin{align}
		\rho_t(g, \bdelta) &\geq \frac{\sigma(\bdelta)^4 \Zbar_{t;ab}^4}{24 B^8} \\
		\sigma_t^2(g, \bdelta) &\geq \frac 12 \cdot\sigma(\bdelta)^2 \Zbar_{t;ab}^2
	\end{align}
\end{lemma}
\begin{proof}
	We first note that by Markov's inequality, we have for any $\alpha > 0$,
	\begin{equation}
		\pp_w\left(\abs{\inprod{\bw}{\bdelta} - \ee_w\left[\inprod{\bw}{\bdelta} > | Z_{t;ab}\right]} > \alpha | Z_{t;ab}\right) \leq \frac{\Varw\left[\inprod{\bw}{\bdelta} | Z_{t;ab}\right]}{\alpha^2}.
	\end{equation}
	Rearranging, we see that
	\begin{align}
		\Varw\left[\inprod{\bw}{\bdelta} | Z_{t;ab}\right] \geq \sup_{\alpha > 0} \alpha^2 \pp_w\left(\abs{\inprod{\bw}{\bdelta} - \ee_w\left[\inprod{\bw}{\bdelta} > | Z_{t;ab}\right]} > \alpha | Z_{t;ab}\right).
	\end{align}
	Now, we compute:
	\begin{align}
		\pp_w\left(\abs{\inprod{\bw}{\bdelta} - \ee_w\left[\inprod{\bw}{\bdelta} > | Z_{t;ab}\right]} > \alpha | Z_{t;ab}\right) &= 1 - \pp_w\left(\abs{\inprod{\bw}{\bdelta} - \ee_w\left[\inprod{\bw}{\bdelta} > | Z_{t;ab}\right]} \leq \alpha | Z_{t;ab}\right) \\
		&= 1 - \frac{1}{\Zbar_{t;ab}} \ee_w\left[\bbI[Z_{t;ab}] \bbI[\abs{\inprod{\bw}{\bdelta} - \ee_w\left[\inprod{\bw}{\bdelta} > | Z_{t;ab}\right]} \leq \alpha]  \right] \\
		&\geq 1 - \frac{1}{\Zbar_{t;ab}} \ee_w\left[\bbI[\abs{\inprod{\bw}{\bdelta} - \ee_w\left[\inprod{\bw}{\bdelta} > | Z_{t;ab}\right]} \leq \alpha]  \right] \\
		&\geq 1 - \frac{t}{\sigma(\bdelta)\Zbar_{t;ab}}
	\end{align}
	Setting $t = \frac{\sigma(\bdelta) \Zbar_{t;ab}}{2}$ and plugging in concludes the proof.
\end{proof}

\subsection{Disagreement Cover. }
\begin{definition}[Disagreement Cover] An $\epsilon$-disagreement cover $\scrD$ of $\Gclass_{\epsilon}$ is a collection of functions $g_i$ and regions $\cD_i \subset \R^d$ such that, 
\begin{itemize}
	\item For every $g \in \Gclass$, there exists $(g_i,\cD_i) \in \scrD$ for which $\{\bx \in \R^d: g_i(\bx) \ne  g(\bx) \} \subset \cD_i$. 
	\item For all $i$, $\sup_{\bz \in \R^d} \Prw[\bz + \bw \in \cD_i] \le \epsilon$.
\end{itemize}
\end{definition}
Note that a disagreement cover is somewhat stronger than a standard cover, as it requires the disagreement of possible multiple functions $g \in \Gclass$ to be contained in one region $\cD_i$. 

\begin{lemma}\label{lem:dis_cover} Let $\scrD = \{(g_i,\cD_i)\}$ be an $\epsilon$-disagreement cover. Then, with probability $1-\delta$,
\begin{align*}
\max_{g \in \Gclass}\min_{g_i} \sum_{t=1}^T\I\{g(\bx_t) \ne g_i(\bx_t)\} \le 2T\epsilon + 6\log(|\scrD|/\delta). 
\end{align*}
\end{lemma}
\begin{proof}  By the definition of a disagreement cover,
\begin{align*}
\max_{g \in \Gclass}\min_{g_i} \sum_{t=1}^T\I\{g(\bx_t) \ne g_i(\bx_t)\}  \le \max_{\cD_i}\sum_{t=1}^T\I\{\bx_t \in \cD_i\} .
\end{align*}
 Observe that $\Pr[\bx_t \in \cD_i \mid \filtz_t] = \Prw[\bz_t + \bw \in \cD_i] \le \sup_{\bz \in \R^d}\Prw[\bz + \bw \in \cD_i] \le \epsilon$, by definition of a disagreement cover. We will use a looser bound $\Pr[\bx_t \in \cD_i \mid \filtz_t] \le \epsilon'$, where $\epsilon' \ge \epsilon$ is a parameter of our choosing. Hence, for a fixed $\cD_i$, a Chernoff bound (\Cref{lem:chernoff}) yields
\begin{align*}
\Pr[\sum_{t=1}^T \I\{\bx \in \cD_i\} \ge 2T\epsilon'] \le \exp(-t\epsilon'/3)
\end{align*}
Taking $\epsilon' = \epsilon + 3\log(1/\delta)$, we have $\Pr[\sum_{t=1}^T \I\{\bx \in \cD_i\} \ge 2T\epsilon + 6\log(1/\delta)] \le \delta.$ The lemma follows from a union bound.

%By associating each $g \in \Gclass$ to the pair $(g_i,\cD_i) \in \scrD$ for which $\{\bx \in \R^d: g_i(\bx) \ne  g(\bx) \} \subset \cD_i$, it suffices to show that 
\end{proof}


\subsection{Regression Notation}

Given $g \in \Gclass$ and iterates $(\bx_1,\by_1),\dots,(\bx_T,\by_T)$,  $\Igab := \{t: g(\bx_t) = a, \gst(\bx_t) = b\}$. We define
\begin{align*}
\Rabst(g) &:= \sum_{t \in \Igab} \|\Thethat_a \cdot \barbx_t - \by_t \|^2 - \|\Thetst_b \cdot \barbx_t - \by_t \|^2 
%&= \sum_{t \in \Igab} \|(\Thethat_a - \Thetst_b) \cdot \barbx_t - \be_t \|^2 - \|\be_t \|^2 \\
%&= \sum_{t \in \Igab} \|(\Thethat_a - \Thetst_b) \cdot \barbx_t\|_2^2 -  2\langle \be_t, (\Thethat_a - \Thetst_b)\bx_t\rangle. 
\end{align*}
Throughout, we assume a known upper bound $R$ on $\fronorm{\Thethat_a},\fronorm{\Thetst_b}$ for all $a,b$. Oracle provides
\begin{align*}
\epsorac &\ge \sum_{t=1}^T \|\Thethat_{\ghat(\bx_t)} \cdot \barbx_t - \by_t \|^2 - \inf_{\tilde g \in \Gclass, \tilde{\boldsymbol \Theta}: \|\tilde{\boldsymbol \Theta}\|_{\fro} \le R} \sum_{t=1}^T\|\tilde{\boldsymbol{\Theta}}_{\tilde g(\bx_t)} \cdot \barbx_t - \by_t \|^2 \\
&\ge \sum_{t=1}^T \|\Thethat_{\ghat(\bx_t)} \cdot \barbx_t - \by_t \|^2 -  \sum_{t=1}^T\|\Thetst_{\gst(\bx_t)} \cdot \barbx_t - \by_t \|^2 = \sum_{a,b = 1}^K \Rabst(\ghat).
\end{align*}



\begin{lemma}\label{lem:Q_lower_bound} Let $\Qab(g) := \sum_{t \in \Igab} \|(\Thethat_a - \Thetst_b) \cdot \barbx_t\|_2^2$. Then, with probability $1-\delta$, the following holds for any fixed $g \in \Gclass$ and all $(a,b) \in [K]^2$ simultaneously:
\begin{align*}
\Rabst(g)  \ge  \Qab(g) - 4\sige\sqrt{(\lambda + \Qab(g))\beta_1(\delta,\lambda)},
\end{align*}
where, for a universal constant $c> 0$, we define $\beta_1(\delta,\lambda) := \log (2K^2/\delta) + cdm\log (\log(K^2/\delta) \cdot M/\lambda)$, for $M :=  TR^2B^2md$.
\end{lemma}


\begin{lemma}
	For fixed $a, b$ and $g$, define $ \Sigma_{ab}(g) :=   \sum_{t \in I_{ab}((g)}\barbx_t \barbx_t^\top$. Then, with probability at least $1 - \delta$, if
% \begin{align}
% 	\abs{I_{ab}(g)} \geq \left(2 \sqrt{T \log\left(\frac 2\delta\right) + \frac {Td}2 \log\left(C\frac{R \sigma^2}\rho\right) }\right) \vee \left(\frac{256}{\rho^2}\left(\log\left(\frac{\log\frac{2T}{\rho}}{\delta}\right) +  \frac d2 \log\left(C\frac{R \sigma^2}\rho\right)\right)^2 \right)
% \end{align}
\begin{align}
	\abs{I_{ab}(g)} \geq \frac{2}{\rho^2} \log\left(\frac{2 T}{\delta}\right) + \frac{d}{\rho^2} \log\left(C\frac{B \sigma^2}{\rho}\right)
\end{align}
then
\begin{align}
     \Sigma_{ab}(g) \succeq \frac{c_0 \sigma^2}{4} \abs{I_{ab}(g)}
\end{align}
\end{lemma}
\begin{proof}
	Note that for any fixed unit vector $v$, the following holds:
	\begin{align}
		\pp\left(v^T \Sigma_{ab}(g) v \leq \frac{c_0 \rho \sigma^2 \abs{I_{ab}(g)}}{2}\right) \leq \pp\left(\sum_{t = 1}^T \bbI\left[v^T x_t x_t^T v \leq c_0 \sigma^2\right] Z_{t;a,b} \leq \frac{\rho \abs{I_{ab}(g)}}{2}\right)
	\end{align}
	Now, using \Cref{lem:small_bal} to control the conditional probability of the event that $v^T x_t x_t^T v \leq c_0 \sigma^2$ and applying \Cref{lem:conditional_smallball} to the above sum, we see that if $\abs{I_{ab}(g)}$ satisfies the bound in the statement, then with probability at least $1 - \delta \exp\left(- \frac d2 \log\left(C\frac{R \sigma^2}\rho\right)\right)$, we have that the desired inequality holds.  Taking a union bound over an appropriately sized $\epsilon$-net and applying \cite[Lemma 45]{block2022efficient} concludes the proof.
\end{proof}


\begin{lemma}
Let $\scrD$ be a disagreement cover.  Then with probability at least $1 - \delta$, for all $a,b,g$ such that
% \begin{align}
% 	\abs{I_{ab}(g)} &\geq \left(2 \sqrt{T \log\left(\frac {2 K^2 \dn(\epsilon)}\delta\right) + \frac {Td}2 \log\left(C\frac{R \sigma^2}\rho\right) }\right) \vee \left(\frac{256}{\rho^2}\left(\log\left(\frac{K^2 \dn(\epsilon)\log\frac{2T}{\rho}}{\delta}\right) +  \frac d2 \log\left(C\frac{R \sigma^2}\rho\right)\right)^2 \right) \\
% 	&\quad \vee \left(C \frac{B}{\sigma^2} (T \epsilon + \log\left(\frac{\dn(\epsilon)}{\delta}\right))\right)
% \end{align}
\begin{align}
	\abs{I_{ab}(g)} \geq \max\left(\frac{2}{\rho^2}\left(\log\left(\frac{2T}{\delta}\right) + \frac d2 \log\left(C \frac{B \sigma^2}{\rho}\right) + \log\left(K^2 \abs{\scrD}\right) \right), C\frac{B}{\sigma^2} \left(2 T \epsilon + 6 \log\left(\frac{\abs{\scrD}}{\delta}\right)\right) \right)
\end{align}
it holds that
\begin{equation}
	\Sigma_{ab}(g) \succeq \frac{c_0 \sigma^2}{8} \abs{I_{ab}(g)}
\end{equation}
\end{lemma}
\begin{proof}
	We begin by noting that a union bound and \Cref{lem:singlefunction_smallball} tell us that with probability at least $1 - \delta$, for all $g_i, a, b$ with sufficiciently large $I_{ab}(g_i)$, it holds simultaneously that
	\begin{equation}
		\Sigma_{ab}(g_i) \succeq \frac{c_0 \sigma^2}{4} \abs{I_{ab}(g_i)}
	\end{equation}
	Note that by \Cref{lem:dis_cover}, with probability at least $1 - \delta$, for every $g \in \G$, there is some $g_i$ in the cover such that the number of $t$ on which $g$ disagrees with $g_i$ is at most $2 T \epsilon + 6 \log\left(\frac{\abs{\scrD}}\delta\right)$.  As $\norm{x_tx_t^T} \leq B$, we have
	\begin{align}
		\Sigma_{ab}(g) \geq \Sigma_{ab}(g_i) - B (2 T \epsilon + 6 \log\left(\frac{\abs{\scrD}}{\delta}\right))
	\end{align}
	Applying the lower bound from \Cref{lem:singlefunction_smallball} and the condition on $\abs{I}_{ab}(g)$ concludes the proof.
\end{proof}
\begin{lemma}\label{lem:parameter_recovery}
	Suppose we are in the situation of \Cref{lem:Q_lower_bound}.  Then with probability at least $1 - \delta$, it holds for all $a, b$ such that $I_{ab}(\widehat{g})$ satisfies the condition in \Cref{lem:uniform_smallball} that
	\begin{align}
		C \sigma^2 \abs{I_{ab}(\widehat{g})} \norm{\widehat{\Theta}_a - \Theta_b^\ast}^2 &\leq 32 \nu^2 \beta_1\left(\frac{\delta}{\dn(\epsilon)}, \lambda\right) + 8\nu \sqrt{2 \beta_1\left(\frac{\delta}{\dn(\epsilon)}, \lambda\right) \lambda}+ \epsorac \\
		&\quad  + 4 B^2 R^2\left(2 T \epsilon + 6 \log\left(\frac{\dn(\epsilon)}{\delta}\right)\right)+ \left(2 B^2 R^2 + \nu^2 \log\left(\frac T\delta\right)\right)\left(2 T \epsilon + \log\left(\frac{\dn(\epsilon)}{\delta}\right)\right)
		\end{align} 
\end{lemma}
\begin{proof}
	By \Cref{lem:Q_lower_bound}, it holds with probability at least $1 - \delta$  for any fixed $g$ that
	\begin{equation}
		\Qab(g) - 4 \nu \sqrt{\lambda + \Qab(g) \beta_1(\delta, \lambda)} \leq \mathcal{R}_{ab}(g)
	\end{equation}
	Rearranging, this implies that for any fixed $g$, with probability at least $1 - \delta$, it holds that
	\begin{equation}
		\Qab(g) \leq 32 \nu^2 \beta_1(\delta, \lambda) + 8 \nu \sqrt{2 \beta_1(\delta, \lambda) \lambda} + \mathcal{R}_{ab}(g)
	\end{equation}
	By \Cref{lem:dis_cover}, with probability at least $1 - \delta$, it holds that
	\begin{align}
		\norm{\Qab(\widehat g) - \Qab(g_i)} \leq 4 B^2 R^2 \left(2 T \epsilon + 6 \log\left(\frac{\dn(\epsilon)}{\delta}\right)\right)
	\end{align}
	and thus it hoolds that with probability at least $1 - 2\delta$,
	\begin{equation}
		\Qab(\widehat g) \leq 32 \nu^2 \beta_1\left(\frac{\delta}{\dn(\epsilon)}, \lambda\right) + 8\nu \sqrt{2 \beta_1\left(\frac{\delta}{\dn(\epsilon)}, \lambda\right) \lambda} + \epsorac + 4 B^2 R^2\left(2 T \epsilon + 6 \log\left(\frac{\dn(\epsilon)}{\delta}\right)\right) + \mathcal{R}_{ab}(g_i) - \mathcal{R}_{ab}(\widehat g)
	\end{equation}
	Note that
	\begin{equation}
		\Qab(g) \geq \lambda_{min}(\Sigma_{ab}(g)) \norm{\widehat{\Theta}_{a} - \Theta_b^\ast}^2
	\end{equation}
	Also note that with probability at least $1 - \delta$, it holds that
	\begin{align}
		\mathcal{R}_{ab}(g_i) - \mathcal{R}_{ab}(\widehat{g}) &= \sum_{t \in I_{ab}(g_i)\setminus I_{ab}(\widehat{g})} \norm{\widehat{\Theta}_a \cdot \barbx_t - \by_t }^2 - \norm{\Theta_b^\ast \cdot \barbx_t - \by_t}^2 - \sum_{t \in I_{ab}(\widehat g)\setminus I_{ab}(g_i)} \norm{\widehat{\Theta}_a \cdot \barbx_t - \by_t }^2 - \norm{\Theta_b^\ast \cdot \barbx_t - \by_t}^2 \\
		&\leq \left(2 B^2 R^2 + \nu^2 \log\left(\frac T\delta\right)\right)\left(2 T \epsilon + \log\left(\frac{\dn(\epsilon)}{\delta}\right)\right)
	\end{align}
	Putting everything together concludes the proof.
\end{proof}
We now put everything together:
\begin{theorem}[Parameter Recovery]
	Suppose we are in the above situation.  Then with probability at least $1 - \delta$, for all $a, b$ such that $\Zbar_{t; ab} \geq \eta$ and 
	\begin{equation}
		\abs{I_{ab}(g)} \geq \max\left(\frac{500}{\sigma^8 \eta^8}\left(\log\left(\frac{2T}{\delta}\right) + \frac d2 \log\left(CB\right) + \log\left(K^4 d^2 T\right) \right), C\frac{B}{\sigma^4 \eta^4} \left(2 + 6 K d^2 \log\left(\frac{KT}{\delta}\right)\right) \right)
	\end{equation}
	it holds for any $\lambda > 0$,
	\begin{align}
		\norm{\widehat{\Theta}_a - \Theta_b^\ast}^2 \lesssim \frac 1{\eta^4 \sigma^4 \cdot \abs{\Igab}} \left(1 + \epsorac + \nu^2 K d^3 m \log\left(\frac{T^2 R^2 B^2 m d K}{\delta}\right) + B^2 R^2 K d^2 (1 + \nu^2) \log^2\left(\frac{KT}{\delta}\right)\right)
	\end{align}
\end{theorem}







\paragraph{Back to proofs}



\begin{proof}[Proof of \Cref{lem:Q_lower_bound}] Fix $a,b \in [K]$. We expand
\begin{align*}
\Rabst(g) &:= \sum_{t \in \Igab} \|\Thethat_a \cdot \barbx_t - \by_t \|^2 - \|\Thetst_b \cdot \barbx_t - \by_t \|^2 \\
&= \sum_{t \in \Igab} \|(\Thethat_a - \Thetst_b) \cdot \barbx_t - \be_t \|^2 - \|\be_t \|^2 \\
&= \underbrace{\sum_{t \in \Igab} \|(\Thethat_a - \Thetst_b) \cdot \barbx_t\|_2^2}_{:=\Qab(g)} -  2\sum_{t\in \Igab}\langle \be_t, (\Thethat_a - \Thetst_b)\bx_t\rangle. \numberthis \label{eq:Rabstg}
\end{align*}
For $\bDelta \in \R^{m \times (d+1)}$, define
\begin{align*}
E(\bDelta) := \sum_{t \in \Igab} \langle \be_t, \bDelta\bx_t\rangle, \quad V(\bDelta) := \sum_{t=1}^T\|\bDelta\barbx_\tau\|_2^2
\end{align*}
Observe that
\begin{align*}
  \left(\sum_{t \in \Igab} -2e \langle \be_t, (\Thethat_a - \Thetst_b)\bx_t\rangle\right)^2&= 4E(\Thethat_a - \Thetst_b)^2 \\
\Qab(g) &= V(\Thethat - \Thetst)
\end{align*}

First, we bound the magnitude of the quantity $E(\bDelta)$ for fixed $\bDelta$, with $\|\bDelta\| \le 2R$.  Let $(\filt_\tau)$ denote the sub-filtration  of $\filtx_t$ stopped at times $\tau$ for which $t \in \Igab$. For such times $\tau$, let $x_\tau := \|\bDelta\barbx_\tau\|_2$, let $\bdelta_\tau$ be any unit vector in the direction of $\bDelta \bx_\tau$ (chosen arbitrarily for $\bDelta \barbx_\tau = 0$) and let $e_\tau = \langle \bdelta_\tau, \be_\tau\rangle $. From \Cref{lem:self_normalized_scalar}, it holds for any fixed $\lambda$ that
\begin{align*}
E(\bDelta)^2 \le 2\sige^2\left(\lambda + V(\bDelta)\right)\log \frac{(1 + \lambda^{-1}\sum_{t=1}^T V(\bDelta))^{1/2}}{\delta}, \quad \text{ w.p. } 1-\delta.
\end{align*} 
By assumption, $\|\barbx_\tau\| \le B$ and $\|\bDelta\|_{\fro} \le 2R$. Hence, $V(\bDelta) \le 4TR^2B^2$. Using $\sqrt{x+y} \le \sqrt{x} + \sqrt{y}$, 
\begin{align*}
E(\bDelta)^2 \le 2\sige^2\left(\lambda + V(\bDelta)\right)\log \frac{1 + 2RB\sqrt{T/\lambda}}{\delta}, \quad \text{ w.p. } 1-\delta.
\end{align*}
Now, let $\scrN_{\epsilon}$ denote a minimal-cardinality $\epsilon$-net of the radius-$2R$ Frobenius ball in $\R^{m \times (d+1)}$, where $\epsilon$ is to be chosen. Then, the following holds with probability $1-\delta$: for any $\bDelta$ of Frobenius norm at most $2R$, and for its nearest-neighbor $\bDelta' \in \scrN$, 
\begin{align*}
E(\bDelta)^2 &= E(\bDelta')^2 + (E(\bDelta)^2 - E(\bDelta)^2)\\
&\le (E(\bDelta)^2 - E(\bDelta')^2) +  2\sige^2\left(\lambda + V(\bDelta')\right)\left(\log \frac{1 + 2RB\sqrt{T/\lambda}}{\delta} + \log |\scrN_{\epsilon}|\right)\\
&\le  2\sige^2\left(\lambda + V(\bDelta)\right)\left(\log \frac{1 + 2RB\sqrt{T/\lambda}}{\delta} + \log |\scrN_{\epsilon}|\right)\\
&\quad+ (E(\bDelta)^2 - E(\bDelta')^2) + 2\sige^2\left(V(\bDelta') - V(\bDelta)\right)\left(\log \frac{1 + 2RB\sqrt{T/\lambda}}{\delta} + \log |\scrN_{\epsilon}|\right)\\
&\le  2\sige^2\left(\lambda + V(\bDelta)\right)\left(\log \frac{1 + 2RB\sqrt{T/\lambda}}{\delta} + (d+1)m\log \frac{10R}{\epsilon}\right)\\
&\quad+ \underbrace{(E(\bDelta)^2 - E(\bDelta')^2) + 2\sige^2\left(V(\bDelta') - V(\bDelta)\right)\left(\log \frac{1 + 2RB\sqrt{T/\lambda}}{\delta} + (d+1)m\log \frac{10R}{\epsilon}\right)}_{E_0},
\end{align*}
where in the last line, we use a standard covering number bound for $\epsilon \le \frac{1}{2}\cdot 2R$
Our aim is to select $\epsilon$ so that the terms on the last line are at most $2\lambda \sige^2  $. Define $\bar{E} := \sum_{t =1}^T \|\be_t\|^2$. Observe that, by Cauchy-Schwartz, $E(\tilde \bDelta)^2 \le \bar{E}\cdot V(\tilde \bDelta)$ for ay $\tilde \bDelta$.
Moreover, since $E(\cdot)$ is a linear function,
\begin{align*}
(E(\bDelta)^2 - E(\bDelta')^2 &= (E(\bDelta) + E(\bDelta'))(E(\bDelta) - E(\bDelta'))\\
&= E(\bDelta + \bDelta') \cdot E(\bDelta - \bDelta')\\
&= \left(\sum_{t \in \Igab} \langle \be_t, (\bDelta+\bDelta')\bx_t\rangle\right)  \left(\sum_{t \in \Igab} \langle \be_t, (\bDelta-\bDelta')\bx_t\rangle\right) \\
&\le  \bar{E} \sqrt{V( \bDelta+\bDelta')}\cdot \sqrt{V(\bDelta - \bDelta')}\\
&\le  \bar{E} \sqrt{16TR^2B^2}\cdot \sqrt{V(\bDelta - \bDelta')}
\end{align*}
Similary, 
\begin{align*}
V(\bDelta') - V(\bDelta) &= \sum_{t \in \Igab} \|\bDelta'\barbx_t\|^2- \|\bDelta\barbx_t\|^2\\
&= \sum_{t \in \Igab} (\|\bDelta'\barbx_t\|+\|\bDelta'\barbx_t\|)( \|\bDelta'\barbx_t\|-\|\bDelta'\barbx_t\|)\\
&\le \sum_{t \in \Igab} (4RB)| \|(\bDelta' - \bDelta')\barbx_t\|\\
&\le \sqrt{16TR^2B^2}\cdot \sqrt{V(\bDelta - \bDelta')}.
\end{align*}
Lastly, $V(\bDelta - \bDelta') = \sum_{t \in \Igab} \|(\bDelta-\bDelta')\barbx_t\|^2 \le \sum_{t \in \Igab} \|(\bDelta-\bDelta')\|_{\op}^2\|\barbx_t\|^2  \le TB^2\|(\bDelta-\bDelta')\|_{\op}^2 \le TB^2\|(\bDelta-\bDelta')\|_{\fro}^2 \le TB^2 \epsilon^2$. Hence,
\begin{align*}
&E_0 := (E(\bDelta)^2 - E(\bDelta')^2) + 2\sige^2\left(V(\bDelta') - V(\bDelta)\right)\left(\log \frac{1 + 2RB\sqrt{T/\lambda}}{\delta} + \log |\scrN_{\epsilon}|\right)\\
&\le  \sqrt{16TR^2B^2}\cdot \sqrt{V(\bDelta - \bDelta')} \left(\bar{E} +  2\sige^2\left(\log \frac{1 + 2RB\sqrt{T/\lambda}}{\delta} + (d+1)m\log\frac{5}{2R\epsilon}\right)  \right)\\
&\le  4TB^2R \epsilon\cdot \left(\bar{E} +  2\sige^2\left(\log \frac{1 + 2RB\sqrt{T/\lambda}}{\delta} + (d+1)m\log\frac{5}{2R\epsilon}\right)  \right).
\end{align*}
To conclude, let us upper bound $\bar{E}$ with probability $1-\delta$, and then select $\epsilon$. Observe that $\bar{E}$ is the squared norm of the vector $\bar{\be}_T := (\be_1,\dots,\be_T)$. Since each component is conditionally $\sige^2$ subGaussian, an MGF computation reveals the entire vector is as well. Hence, for any fixed $\bar{\bv} = (\bv_1,\dots,\bv_T)$ of norm $1$, $\langle \bar{\be}_T, \bar \bv \rangle \le \sqrt{2\sige^2\log(1/\delta)}$. By a standard covering argument (noting $\dim(\bar \bv) = Tm$), we have $\bar E = \|\bar{\be}_T\|^2 \le 2\sige^2(Tm\log 5 + \log(1/\delta))$ . Thus, with probability $1 - 2\delta$,
\begin{align*}
E_0 &\le  2\sige^2 \cdot 4TB^2R \epsilon\cdot \left(Tm\log 5 + 2\log(1/\delta) + \left(\log (1 + 2RB\sqrt{T/\lambda}) + (d+1)m\log\frac{10R}{\epsilon}\right)  \right)\\
&\le   2\sige^2 \lambda \cdot \epsilon \cdot \frac{4TB^2R}{\lambda} \cdot \left(Tm\log 5 + 2\log(1/\delta) +  2RB\sqrt{T/\lambda} + (d+1)m\log\frac{10R}{\epsilon}\right)  
\end{align*}
By choosing $\epsilon = \left(c_1 + c_2(\log(1/\delta) \cdot TR^2B^2md/\lambda)^{-c_3}\right)$ for universal constants $c_1,c_2,c_3>0$, the above can be made to at most $2\sige^2 \lambda$. With this choice, it holds with probability $1- 2\delta$, that for all $\bDelta:\|\bDelta\|_{\fro} \le 2R$,
\begin{align*}
E(\bDelta)^2 &=   2\sige^2\left(2\lambda + V(\bDelta)\right)\left(\log \frac{1 + 2RB\sqrt{T/\lambda}}{\delta} + c'(d+1)m\log (\log(1/\delta) \cdot 1+TR^2B^2md/\lambda)\right)\\
&\le  2\sige^2\left(2\lambda + V(\bDelta)\right)\left(\log (1/\delta) + c''dm\log (\log(1/\delta) \cdot M/\lambda)\right) \\
%&:= 2\sige^2(2\lambda + V(\bDelta) + \beta_1(\delta,\lambda)).
\end{align*}
where $M := TR^2B^2md$. Reparameterizing $\delta \gets \delta/2K^2$, we can take
\begin{align*}
E(\bDelta)^2  \le 2\sige^2(2\lambda + V(\bDelta)) \beta_1(\delta,\lambda) \quad \text{w.p. } 1- \delta/K^2,
\end{align*}
where $\beta_1(\delta,\lambda) = \log (2K^2/\delta) + cdm\log (\log(K^2/\delta) \cdot M/\lambda)$ for some universal $c>0$.In particular, under the assumption that $\|\Thethat_a\|_{\fro}\vee \|\Thetst_b\|_{\fro} \le R$, it holds with probability $1-\delta/K^2$
\begin{align*}
\left(-2\sum_{t \in \Igab} \langle \be_t, (\Thethat_a - \Thetst_b)\bx_t\rangle\right)^2  &= 4E(\Thethat - \Thetst)^2 \\
&\le 8\sige^2(2\lambda + V(\Thethat_a - \Thetst_b)) \beta_1(\delta,\lambda) \\
&=  8\sige^2(2\lambda + \Qab(g)) \beta_1(\delta,\lambda).
\end{align*}
Thus, from \eqref{eq:Rabstg}, we conclude, 
\begin{align*}
\Rabst(g) \ge \Qab(g) - 4\sige\sqrt{(\lambda + \Qab(g))\beta_1(\delta,\lambda)}.
\end{align*}
\end{proof}





\section{Proofs}

\subsection{Proof of Lemma \ref{lem:small_bal}}
	\begin{lemma}\label{lem:var_lb} Then, for any $\barbv \in S^d$ with $\bv \ne 0$,
	\begin{align*}
	\Exp[\langle \barbx_t, \barbv \rangle^2 \mid \Ztij =1, \filtz_t] 
		&\ge   \zeta_t(\bdelta) :=  \frac{\Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]}{2\vee 12\left(\langle \bz_t, \bdelta\rangle^2 +   \Expw[\langle \bw, \bdelta \rangle ^2\mid \bw \in \Wtab]\right)}. 
	\end{align*}
	where $\bmu_t := \Expw[\bw \mid \bw \in \Wtab]$ and $\bdelta = \bv/\|\bv\|$.
	\end{lemma}
	\begin{proof}[Proof of \Cref{lem:var_lb}] 
		Let $\Wtab := \{\bw: \gst(\bz_t + \bw_t) = a, \ghat(\bz_t + \bw_t) = b\}$. We see that $\Wtab \in \disg$. Note furhter that $\Ztij = 1$ if and only if $\bw_t \in \Wtab$. Hence, defining $\bmu_t := \Expw[\bw \mid \bw \in \Wtab]$, we $\Exp[\bx_t \mid \filtz_t, \Ztij = 1] = \bz_t + \bmu_t$. Then, 
		\begin{align*}
		\Exp[\langle \barbx_t, \barbv \rangle^2 \mid \Ztij =1, \filtz_t] &= \Exp[(v_0 + \langle \bx_t, \bv \rangle)^2 \mid \Ztij =1, \filtz_t] \\
		&\ge \Var[v_0 + \langle \bx_t, \bv \rangle \mid \Ztij =1, \filtz_t] \\
		&=  \Var[(v_0 + \langle \bz_t , \bv \rangle + \langle \bw_t, \bv \rangle) \mid \Ztij =1, \filtz_t] \\
		&=  \Var[\langle \bw_t, \bv \rangle
		 \mid \Ztij =1, \filtz_t] \\
		&=\|\bv\|^2 \Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]. 
		\end{align*}
		We now derive a second lower bound.  Using the elementary inequality $(x+y)^2 \ge x^2/2 - y^2$,
		\begin{align*}
		\Exp[\langle \barbx_t, \barbv \rangle^2 \mid \Ztij =1, \filtz_t] &= \Exp[(v_0 + \langle \bx_t, \bv \rangle)^2 \mid \Ztij =1, \filtz_t] \\
		&\ge \frac{v_0^2}{2} - \Exp[ \langle \bx_t, \bv \rangle^2 \mid \Ztij =1, \filtz_t] \\
		&= \frac{v_0^2}{2} - \Exp[ \langle \bz_t + \bw_t, \bv \rangle^2 \mid \Ztij =1, \filtz_t] \\
		&\ge \frac{v_0^2}{2} -  2\|\bv\|^2\left(\langle \bz_t, \bdelta\rangle^2   + \Exp[ \langle \bw_t , \bdelta \rangle^2 \mid \Ztij =1, \filtz_t]\right) \\
		&\ge \frac{v_0^2}{2} -  2\|\bv\|^2\left(\langle \bz_t, \bdelta\rangle^2 +  + \Expw[\langle \bw, \bdelta \rangle^2 \mid \bw \in \Wtab] \right).
		\end{align*}
		We now combine the two lower bounds. 
		Adopt the shorthand $r := \left(\langle \bz_t, \bdelta\rangle^2 +  + \Expw[\langle \bw, \bdelta \rangle^2 \mid \bw \in \Wtab] \right)/\Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]$. Then, 
		\begin{align*}
		&\Exp[\langle \barbx_t, \barbv \rangle^2 \mid \Ztij =1, \filtz_t] \\
		&\ge \max\{\|\bv\|^2 \Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab], \frac{v_0^2}{2} -  2r\|\bv\|^2 \Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]\}\\
		&\ge \max_{\alpha \in [0,1]} (1-\alpha) \|\bv\|^2 \Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]  + \alpha\left(\frac{v_0^2}{2} -  2r\|\bv\|^2 \Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]\right)\\
		&= \max_{\alpha \in [0,1]} (1-\alpha - 2r\alpha) \|\bv\|^2 \Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]  +\alpha \frac{v_0^2}{2}. 
		\end{align*}
		As $r \ge 1$, we have $(1-\alpha - 2r\alpha)  \ge 1 - 3\alpha r$, so setting $\alpha = 1/6r$, we conclude
		\begin{align*}
		\Exp[\langle \barbx_t, \barbv \rangle^2 \mid \Ztij =1, \filtz_t] &\ge (\|\bv\|^2 + \|\bv_0\|^2)  \min\{\frac{1}{2}\Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab], \frac{1}{12r}\}\\
		&= \|\barbv\|^2   \min\{\frac{\Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]}{2}, \frac{\Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]}{12\left(\langle \bz_t, \bdelta\rangle^2 +   \Expw[\langle \bw, \bdelta \rangle ^2\mid \bw \in \Wtab]\right)}\}\\
		&\ge\underbrace{\|\barbv\|^2}_{=1}   \frac{\Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]}{2\vee 12\left(\langle \bz_t, \bdelta\rangle^2 +   \Expw[\langle \bw, \bdelta \rangle ^2\mid \bw \in \Wtab]\right)}. 
		\end{align*}
		\end{proof}

	\begin{lemma}
	\label{lem:quad_ub} Under the same setup as \Cref{lem:var_lb},
	\begin{align*}
	\Exp[\langle \barbx_t,\barbv \rangle^4 \mid \filtz_t, ~\Ztij = 1] &\le 27  + 27 \langle \bdelta, \bz_t \rangle^4 + 27 \Expw[\langle \bw,\bdelta \rangle^4 \mid \bw \in \Wtab]
	\end{align*}
	\end{lemma}

	\begin{proof}[Proof of \Cref{lem:quad_ub}] We have
	\begin{align*}
	\Exp[\langle \barbx_t,\barbv \rangle^4 \mid \filtz_t, ~\Ztij = 1] &= \Exp[(v_0 + \langle \bx_t,\bv \rangle)^4\mid \filtz_t, ~\Ztij = 1 ]\\
	 &= \Exp[(v_0 +\langle \bw_t, \bv \rangle + \langle \bz_t,\bv \rangle)^4\mid \filtz_t, ~\Ztij = 1 ]
	\end{align*}
	Now, we note that Jensen's inequality gives $(\frac{x+y+z}{3})^4 \le \frac{x^3+y^3+z^3}{3}$, so that $(x+y+z)^4 \le 27(x^4+y^4+z^4)$. Using this fact and the fact that $\bz_t$ is $\filtz_t$-measurable,
	\begin{align*}
	\Exp[\langle \barbx_t,\barbv \rangle^4 \mid \filtz_t, ~\Ztij = 1] &\le 27 v_0^2 + 27 \langle \bv, \bz_t \rangle^4 + 27 \Exp[\langle \bw_t,\bv \rangle^4 \mid \filtz_t, ~\Ztij = 1] \\
	&= 27 v_0^2 + 27 \langle \bv, \bz_t \rangle^4 + 27 \Expw[\langle \bw,\bv \rangle^4 \mid \bw \in \Wtab],
	\end{align*}
	where $\Wtab$ is the same set as in the \Cref{lem:var_lb}. Using that $v_0^2 + \|\bv\|^2 = \|\barbv\|^2 \le 1$, the above is at most
	\begin{align*}
	\Exp[\langle \barbx_t,\barbv \rangle^4 \mid \filtz_t, ~\Ztij = 1] &\le 27  + 27 \langle \bdelta, \bz_t \rangle^4 + 27 \Expw[\langle \bw,\bdelta \rangle^4 \mid \bw \in \Wtab]
	\end{align*}
	where $\bdelta$ is as in \Cref{lem:var_lb}: that is, $\bdelta := \bv/\|\bv\|$.
	\end{proof}



	\begin{proof}[Proof of \Cref{lem:small_bal}] Introduce $\sigma^2 := \Exp[\langle \barbx, \barbv \rangle^2 \mid \Ztij = 1, \filtz_t]$. 
	 By the Paley-Zygmud inequality and \Cref{lem:quad_ub,lem:var_lb},
	\begin{align*}
	\Pr\left[\langle \barbx_t, \barbv \rangle^2 \ge \frac{\sigma^2}{2} \mid \Ztij, ~\filtz_t\right] &\ge \frac{\sigma^4}{4\Exp[\langle \barbx_t,\barbv \rangle^4 \mid \filtz_t, ~\Ztij = 1]}\\
	&\ge  \left(\frac{\Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]}{2\vee 12\left(\langle \bz_t, \bdelta\rangle^2 +   \Expw[\langle \bw, \bdelta \rangle ^2\mid \bw \in \Wtab]\right)}\right)^2  \\
	&\qquad\times \frac{1}{27  + 27 \langle \bdelta, \bz_t \rangle^4 + 27 \Expw[\langle \bw,\bdelta \rangle^4 \mid \bw \in \Wtab]}\\
	&\gtrsim \frac{1 \vee \Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]^2}{\left(1+ \langle \bz_t, \bdelta\rangle^4 +  \Expw[\langle \bw, \bdelta \rangle ^2\mid \bw \in \Wtab]^2\right)(1 +  \langle \bdelta, \bz_t \rangle^4 +  \Expw[\langle \bw,\bdelta \rangle^4 \mid \bw \in \Wtab])}\\
	&\ge \frac{1 \vee \Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]^2}{(1 +  \langle \bdelta, \bz_t \rangle^4 +  \Expw[\langle \bw,\bdelta \rangle^4 \mid \bw \in \Wtab])^2} := \rho_t(\bdelta)
	\end{align*}
	where in the last line, we use Jensen's inequality: $\Expw[\langle \bw,\bdelta \rangle^4 \mid \bw \in \Wtab] \ge \Expw[\langle \bw, \bdelta \rangle ^2\mid \bw \in \Wtab]^2$. Defining 
	\begin{align*}
	\zeta_t^2(\bdelta) := \frac{\Varw[\langle \bw, \bdelta \rangle \mid \bw \in \Wtab]}{1\vee \left(\langle \bz_t, \bdelta\rangle^2 +   \Expw[\langle \bw, \bdelta \rangle ^2\mid \bw \in \Wtab]\right)},
	\end{align*}
	we conclude that there are universal constants $c_1,c_2$ for which
	\begin{align*}
	\Pr\left[\langle \barbx_t, \barbv \rangle^2 \ge c_0\zeta_t^2(\bdelta)\mid \Ztij, ~\filtz_t\right] \ge c_1 \rho_t(\bdelta).
	\end{align*}
	\end{proof}

\section{Technical Lemmas}

\begin{lemma}[Chernoff Bound]\label{lem:chernoff} Let $X_1,\dots,X_t$ be a sequence of binary random variables such that $\Exp[X_i \mid X_{1},\dots,X_{i-1}] \ge \eta$. Then, 
\begin{align*}
\Pr\left[\sum_{i=1}^t X_i \le t\eta/2\right]\le \exp(-t\eta/8)\\
\end{align*}
Similarly,  if $\Exp[X_i \mid X_{1},\dots,X_{i-1}] \le \eta$,
\begin{align*}
\Pr\left[\sum_{i=1}^t X_i \le 2t\eta\right]\le \exp(-t\eta/3)
\end{align*}
\end{lemma}

\begin{lemma}[Freedman's Inequality]\label{lem:freedman}
	Let $(M_t)$ be a martingale with respect to $\filt_t$ and suppose that the martingale difference sequence is uniformly bounded in absolute value by 1.  Let
	\begin{equation}
		\langle M \rangle_T = \sum_{t = 1}^T \ee\left[(M_t - M_{t-1})^2 | \filt_{t-1}\right]
	\end{equation}
	Then for any $x, y > 0$,
	\begin{equation}
		\pp\left(\abs{M_T} \geq x \text{ and } \langle M \rangle_T < y\right) \leq 2 e^{- \frac{x^2 / 2}{y + x/3}}
	\end{equation}
\end{lemma}

We follow \cite{block2021majorizing} and prove a relatex self-normalized bound:
\begin{lemma}[Self-Normalized Martingale Inequality] \label{lem:self_normalized}
	Let $(M_t)$ be a martingale with respect to $\filt_t$ and suppose that the martingale difference sequence is uniformly bounded in absolute value by 1.  Let
	\begin{equation}
		\langle M \rangle_T = \sum_{t = 1}^T \ee\left[(M_t - M_{t-1})^2 | \filt_{t-1}\right]
	\end{equation}	
	Then with probability at least $1 - \delta$, the following inequality holds:
	\begin{equation}
		\abs{M_T} \leq 4 \log\left(\frac{\log\left(\frac T{\langle M \rangle_T}\right)}{\delta}\right)\left(1 + \sqrt{\langle M \rangle_T}\right)
	\end{equation}
\end{lemma}
\begin{proof}
	By \ref{lem:freedman} it holds that for any $x, y$, with probability at least $1 - \delta$ if
	\begin{equation}
		\langle M \rangle_T \leq y
	\end{equation}
	then
	\begin{equation}
		\abs{M_T} \leq \frac 13 \log \left(\frac 2\delta\right) + \sqrt[]{\left(\frac 13 \log\left(\frac 2\delta\right)\right)^2 + 2 y \log\left(\frac 2\delta\right)} \leq 4 \log\left(\frac{\pi^2}{6 \delta}\right)\left(1 + \sqrt{\frac 12 \langle M \rangle_T}\right)
	\end{equation}
	Let $y_j = 2^{-j} T$ and $\delta_j = \frac \delta{j^2}$.  Note that if $\langle M \rangle_j \leq y_j$ then $j \leq \log\left(\frac T{\langle M \rangle_T}\right)$.  A union bound and the preceding display concludes the proof.
\end{proof}
\begin{lemma}[Conditional Small Ball] \label{lem:conditional_small_ball}
	Let $\filt_t$ be a filtration and suppose that events $A_t, B_t \in \filt_t$ for all $t$.  Let
	\begin{align}
		p_{A_t} = \pp\left(A_t | \filt_{t-1}, \, B_t\right) && p_{B_t} = \pp\left(B_t | \filt_{t-1}\right)
	\end{align}
	and suppose that $p_{A_t} \geq \rho$ for all $t$.  Then the following holds:
	\begin{align}
		\pp\left(\sum_{t = 1}^T \bbI[B_t] \geq \left(2 \sqrt{T \log\left(\frac 2\delta\right)}\right) \vee \left(\frac{256}{\rho^2}\left(\log\left(\frac{\log\frac{2T}{\rho}}{\delta}\right)^2\right) \right) \text{ and } \sum_{t  = 1}^T \bbI[A_t] \bbI[B_t] < \frac \rho2 \sum_{t = 1}^T \bbI[B_t] \right) \leq \delta
	\end{align}
\end{lemma}
\begin{proof}
	Let
	\begin{align}
		M_t = \sum_{s = 1}^t (\bbI[A_t] - p_{A_t}) \bbI[B_t] && \langle M \rangle_t = \sum_{s = 1}^T p_{A_t} (1 - p_{A_t}) p_{B_t}
	\end{align}
	Note that $M_t$ is a martingale.  Further note that
	\begin{equation}
		\rho \sum_{t = 1}^T p_{B_t} \leq \langle M \rangle_T \leq \sum_{t = 1}^T p_{B_t}
	\end{equation}
	With probability at least $1 - \delta$, it holds that
	\begin{equation}
		\sum_{t = 1}^T \bbI[B_t] - \sqrt{T \log\left(\frac 2\delta\right)} \leq \sum_{t = 1}^T p_{B_t} \leq \sum_{t = 1}^T \bbI[B_t] + \sqrt{T \log\left(\frac 2\delta\right)}
	\end{equation}
	Applying  \Cref{lem:self_normalized} and rearranging concludes the proof.
\end{proof}


\section{Small Ball with Abbasi-Yadkori Bound}

We begin with the scalar case of \cite[Theorem 1]{abbasi2011improved}
\begin{lemma}[Self-Normalized Martingale Inequality, scalar] 
	Let $(x_t)$ be predictable with respect to a filtration $(\filt_t)$, and let $(e_t)$ be such that $e_t \mid \filt_t$ is $\sige^2$-subGaussian. Then, for any fixed parameter $\lambda> 0$, with probability $1 - \delta$,
	\begin{align*}
	\left(\sum_{t=1}^T x_t e_t\right)^2 \le 2\sige^2\left(\lambda + \sum_{t=1}^T x_t^2\right)\log \frac{(1 + \lambda^{-1}\sum_{t=1}^T x_t^2)^{1/2}}{\delta}
	\end{align*}
	\end{lemma}

\begin{lemma}
	Let $\filt_t$ be a filtration with $A_t \in \filt_t$ and $B_t \in \filt_{t-1}$ for all $t$.  Let
	\begin{align}
		p_{A_t} = \pp\left(A_t | \filt_{t-1}, \, B_t\right) && p_{B_t} = \pp\left(B_t | \filt_{t-1}\right)
	\end{align}
	and suppose that $p_{A_t} \geq \rho$ for all $t$.  Then, with probability at least $1 - \delta$,
	\begin{equation}
		\sum_{t = 1}^T \bbI[A_t] \bbI[B_t] \geq \rho \sum_{t = 1}^T \bbI[B_t] - \frac 12 \sqrt{2 \left(\sum_{t= 1}^T \bbI[B_t]\right) \log\left(\frac{2T}{\delta}\right)}
	\end{equation}
	In particular with probability at least $1 - \delta$, if
	\begin{equation}
		\sum_{t = 1}^T \bbI[B_t] \geq \frac{2}{\rho^2} \log\left(\frac{2 T}{\delta}\right)
	\end{equation}
	then
	\begin{equation}
		\sum_{t = 1}^T \bbI[A_t] \bbI[B_t] \geq \frac{\rho}{2} \sum_{t = 1}^T \bbI[B_t]
	\end{equation}
\end{lemma}
\begin{proof}
	We apply \Cref{lem:self_normalized_scalar} with $x_t = \bbI[B_t]$ and $e_t = \bbI[A_t] - p_{A_t}$.  Noting that the latter is $\frac 18$-subGaussian because it is conditionally mean zero and bounded in absolute value by $1$, we have with probability at least $1 - \delta$,
	\begin{align}
		\abs{\sum_{t = 1}^T (\bbI[A_t] - p_{A_t}) \bbI[B_t]} \leq \frac 12 \sqrt{\left(\lambda + \sum_{t = 1}^T \bbI[B_t]\right)\log\left(\frac{\sqrt{1 + \frac{\sum_{t =1}^T \bbI[B_t]}{\lambda}}}{\delta}\right)}
	\end{align}
	Taking a union bound over $\lambda \in [T]$ and noting that $\sum_{t = 1}^T \bbI[B_t] \in [T]$ almost surely, we recover the result.
\end{proof}


\section{Disagreement Covers}
In this section we prove two lemmas that, together, bound the size of a disagreement cover for the classes of interest.  To begin, we have:
\begin{lemma}
	Let $\G_1, \dots, \G_K$ be function classes mapping $\cX \to \cY$.  Let $h : \cY^{\times K} \to \rr$ be some aggregating function and define
	\begin{equation}
		\G = \left\{x \mapsto h(g_1(x), \dots, g_K(x))| g_1 \in \G_1, \dots, g_K \in \G_K\right\}
	\end{equation}
	Let $\dn(\G_i, \epsilon)$ be the minimal size of an $\epsilon$-disagreement cover of $\G_i$.  Then 
	\begin{equation}
		\dn(\G, \epsilon) \leq \prod_{i = 1}^K \dn\left(\G_i, \frac \epsilon K\right)
	\end{equation}
\end{lemma}
\begin{proof}
	Suppose that $\scrD_i$ are $\left(\frac \epsilon K\right)$-disagreement covers for $\G_i$ and for any $g_i \in \G_i$ denote by $(\pi(g_i), \cD_i(g_i))$ the pair of functions and disagreement sets satisfying the definition of a disagreement cover.  Then we claim that
	\begin{equation}
		\scrD = \left\{\left(h(g_1, \dots, g_K), \bigcup_i \cD_i  \right) | (g_i, \cD_i) \in \scrD_i \right\}
	\end{equation}
	is an $\epsilon$-disagreement cover for $\G$.  Note that $\abs{\scrD}$ is clearly bounded by the desired quantity so this claim suffices to prove the result.

	To prove the claim we first note that a union bound ensures that $\bigcup_i \cD_i$ has an appropriately bounded measure.  We further note that if $g = h(g_1, \dots, g_K)$ then
	\begin{align}
		\left\{x | g \neq h(\pi(g_1), \dots, \pi(g_K))\right\} &\subset \bigcup_{1 \leq i \leq K} \left\{x | g_i \neq \pi(g_i) \right\} \subset \bigcup_{1 \leq i \leq K} \cD_i(g_i).
	\end{align}
	The result follows.
\end{proof}
We now bound the size of a disagreement cover of the class of linear thresholds.
\begin{lemma}\label{lem:lineardisagreementcover}
	Let $\cG : \rr^d \to \{\pm 1\}$ be the class of functions of the form $x \mapsto \sign(\inprod{w}{x})$ for $w \in S^{d-1}$.  Then
	\begin{equation}
		\dn(\G, \epsilon) \leq 4^{d^2} \epsilon^{-d}
	\end{equation}
\end{lemma}
\begin{proof}
	We begin by fixing some $w_i \in S^{d-1}$ and letting $B_i$ denote the geodesic ball of radius $\theta$ around $w_i$, i.e.,
	\begin{equation}
		B_i = \left\{w \in S^{d-1} | \inprod{w}{w'} \leq \cos (\theta) \right\}
	\end{equation}
	We observe that $B_i$ is convex.  Now let $w \in B_i$ and let
	\begin{equation}
		D_i(w) = \left\{x \in S^{d-1} | \sign(\inprod{w}{x}) \neq \sign(\inprod{w_i}{x})\right\}
	\end{equation}
	By the intermediate value theorem, for all $x \in D_i(w)$, there exists some $w_t \in B_i$ such that $\inprod{w_t}{x} = 0$.  Thus, let
	\begin{equation}
		\cD_i = \left\{x \in S^{d-1} | \inprod{w}{x} = 0 \text{ for some } w \in B_i\right\}
	\end{equation}
	Now, by \citet[Corollary 3.18]{gray2003tubes}, because the unit sphere has constant sectional curvature of 1, it holds that for any $\theta \leq \pi$, 
	\begin{equation}
		\vol_{d-1}(B_i) = \frac{2 \pi^{\frac{d - 1}{2}}}{\Gamma\left(\frac{d-1}{2}\right)} \int_0^\theta (\sin t)^{d-2} d t
	\end{equation}
	Thus, in particular, for $\theta \leq \frac \pi 2$, it holds that
	\begin{equation}
		\frac{4 \pi^{\frac{d-1}{2}}}{\Gamma\left(\frac{d-1}{2}\right)(d-1)}\left(\frac \theta 2\right)^{d-1} \leq \vol_{d-1}(B_i) \leq \frac{2 \pi^{\frac{d-1}{2}}}{\Gamma\left(\frac{d-1}{2}\right)(d-1)} \theta^{d-1}
	\end{equation}
	By packing-covering duality and the fact that $\vol_{d-1}(S^{d-1}) = \frac{2 \pi^{\frac d2}}{\Gamma\left(\frac{d}{2}\right)}$, it holds that for the appropriate choices of $w_i$, we can form an $\epsilon$-disagreement cover of size
	\begin{equation}
		\dn(\G, \epsilon) \leq \frac{d-1}{2} \sqrt{\pi} \left(\frac{\theta}{4}\right)^{- (d - 1)}
	\end{equation}
	where $\epsilon$ is the measure of $\cD_i$.  Now, we note that $\cD_i$ is contained in the tube of radius $\theta$ around the equator of $S^{d-1}$ orthogonal to $w_i$, by \citet[Lemma 28]{block2022efficient}.  Now, by the generalized Steiner formula \citep[Theorem 10.20 (ii)]{gray2003tubes}, and the fact that the sphere has constant mean curvature, it holds that
	\begin{align}
		\vol_{d-1}(\cD_i) \leq \int_0^\theta \int_{S^{d-2}} (1 + t)^{d-2} d \vol_{d-2}(\cdot) d t \leq 2^{d-2} \vol_{d-2}(S^{d-2}) \theta
	\end{align}
	After normalizing by $\vol_{d-1}(S^{d-1})$, we get that
	\begin{equation}
		\mu(\cD_i) \leq 2^{d-3} \frac{d-1}{\sqrt{\pi}} \theta
	\end{equation}
	Setting $\theta$ small enough to ensure that $\mu(\cD_i) \leq \epsilon$ concludes the proof.
\end{proof}
As an immediate corollary, we have the following result:
\begin{corollary}\label{cor:disagreementcoversize}
	Let $\G$ be a class of multi-class classifiers given by an aggregating function of $K$ linear thresholds.  Then
	\begin{equation}
		\log(\dn(\G, \epsilon)) \leq K d^2 \log\left(\frac{4 K}{\epsilon}\right)
	\end{equation}
\end{corollary}
\begin{proof}
	Combine \Cref{lem:disagreement1,lem:lineardisagreementcover}.
\end{proof}

==> body/online_learning_old.tex <==
\section{Online Learning}
\subsection{A schematic result}
We have sequence of feature-label pairs $z_i^\star (x_i,y_i^\star)_{1 \le i \le T}$. For each epoch $k$, we have a classifier $\hat g _k $.  Let $k(i)$ denote an epoch associated with time index $i$, and define
\begin{align*}
    \hat z_i := (x_i, \hat{y}^i_\star), \quad \hat{y}^i_{\star}  := \hat{g}_{k(i)}(x_i). 
\end{align*}
Introduce the losses
\begin{align*}
\tilde{\ell}_{\gamma,t}(w) &:= \max\{0,1 - \gamma^{-1}\hat{y}_t\langle w, x_t \rangle  \}\\
\tilde w_t &:= \Pi_{\cK}\left(\tilde w_{t-1} - \eta \nabla \tilde{\ell}_{\gamma,t-1}(w_{t-1})\right)\\
\hat{w}_{t;m} &\in \{\tilde{w}_t, \tilde{w}_{t-1}, \dots, \tilde{w}_{t-m+1}\}
\end{align*}
Then, 
\begin{align*}
\hat{\ell}_{\mathtt{01},t}(w) &:= \I\{\sign(\langle w, x_t \rangle ) \ne \hat{y}_t\}\\
\ell_{\mathtt{01},t}^\star(w) &:= \I\{\sign(\langle w, x_t \rangle ) \ne y^\star_t\}\\
\bar\ell_{\mathtt{01},t}^\star(w) &:= \Exp[\ell_{\mathtt{01},t}^\star(w) \mid \cF_{t-1}]  \text{ under smoothing}
\end{align*}
Let 
\begin{align*}
\sum_{t=1}^T \ell^{\star}_{\mathtt{01},t}(\hat{w}_{t;m}) &= \text{(martingale)} + \sum_{t=1}^T \bar\ell^{\star}_{\mathtt{01},t}(\hat{w}_{t;m})\\
&\le \text{(martingale)} +  \mathrm{Lip}(\bar\ell^{\star}) \cdot \sum_{t=1}^T \|\tilde{w}_t - \hat{w}_{t;m}\| + \sum_{t=1}^T \bar\ell^{\star}_{\mathtt{01},t}(\hat{w}_{t})\\
&\le \text{(martingale)} +  \mathrm{Lip}(\bar\ell^{\star}) \cdot Tm \eta + \sum_{t=1}^T \bar\ell^{\star}_{\mathtt{01},t}(\hat{w}_{t})\\
&\le 2*\text{(martingale)} +  \mathrm{Lip}(\bar\ell^{\star}) \cdot Tm \eta + \sum_{t=1}^T \ell^{\star}_{\mathtt{01},t}(\hat{w}_{t}) \tag{additive subtracting martingale diff}\\
&\le 2*\text{(martingale)} +  \mathrm{Lip}(\bar\ell^{\star}) \cdot Tm \eta  + \sum_{t=1}^T\I\{\hat{y}_t \ne y^\star_t\} + \sum_{t=1}^T \hat\ell_{\mathtt{01},t}(\hat{w}_{t})\\
&\le 2*\text{(martingale)} +  \mathrm{Lip}(\bar\ell^{\star}) \cdot Tm \eta  + \sum_{t=1}^T\I\{\hat{y}_t \ne y^\star_t\} + \sum_{t=1}^T \tilde\ell_{\gamma,t}(\hat{w}_{t}) \tag{0,1 less than hinge}\\
&\le 2*\text{(martingale)} +  \mathrm{Lip}(\bar\ell^{\star}) \cdot Tm \eta  + \sum_{t=1}^T\I\{\hat{y}_t \ne y^\star_t\} + \mathrm{RegretTerm}_T +  \inf_{w_0}\sum_{t=1}^T \tilde\ell_{\gamma,t}(w_0) \tag{0,1 less than hinge}
\end{align*}
This has to be bounded using separation. 
\begin{align*}
    \sum_{t=1}^T\I\{\hat{y}_t \ne y^\star_t\} = \sum_{k} \sum_{t:k(t) = k} \I\{\hat{g}_{k+1}(x_t) \ne g^\star(x_t)\}
\end{align*}
\begin{lemma} Suppose $\|w\| \le 1$. $\tilde\ell_{\gamma,t}(w_0) \le \I\{\text{no margin } \gamma\} + \gamma^{-1}\hat{\ell}_{\mathtt{01},t}$.
\end{lemma}
\begin{proof} We have two cases. In case 1, $\hat{\ell}_{\mathtt{01},t} = 0$. Then, the only time you make a make a loss is if the margin is less than $\gamma$. Otherwise, $\hat{\ell}_{\mathtt{01},t} = 1$. In which case $\tilde{\ell}_{\gamma,t}(w_0) \le \gamma^{-1} =\gamma^{-1} \hat{\ell}_{\mathtt{01},t}$.
\end{proof}


Similarly, 
\begin{align*}
 \inf_{w_0}\sum_{t=1}^T \tilde\ell_{\gamma,t}(w_0) &\le \sum_{t=1}^T \I\{\text{no margin } \gamma\} + \gamma^{-1}\inf_{w_0}\sum_{t=1^T}\hat\ell_{\mathtt{01},t}(w_0)\\
 &\le \sum_{t=1}^T \I\{\text{no margin } \gamma\} + \gamma^{-1}\sum_{t=1}^T\I\{\hat{y}_t \ne y^\star_t\} + \underbrace{\inf_{w_0}\sum_{t=1}^T\ell^\star_{\mathtt{01},t}(w_0)}_{=0},
\end{align*}
where the last thing is zero due to realizabilty. Ultimately, one has
\begin{align*}
    &\sum_{t=1}^T \ell^{\star}_{\mathtt{01},t}(\hat{w}_{t;m}) \\
    &\le  2*\text{(martingale)} +  \mathrm{Lip}(\bar\ell^{\star}) \cdot Tm \eta  + (1+\gamma^{-1}) \sum_{t=1}^T\I\{\hat{y}_t \ne y^\star_t\} + \sum_{t=1}^T \I\{\text{no margin } \gamma\} + \mathrm{RegretTerm}_T 
\end{align*}
Here, $\mathrm{Lip}(\bar\ell^{\star}) $ should just be directional smoothness. 

\subsection{Lemmas for Online Learning Section}
In this section, we use the notation introduced in the preceding section:
\begin{lemma}\label{lem:martingalepart}
    With probability at least $1 - \delta$, the following inequalities hold:
    \begin{align}
        \sum_{t = 1}^T \ell^{\star}_{\mathtt{01},t}(\hat{w}_{t;m}) - \bar\ell^{\star}_{\mathtt{01},t}(\hat{w}_{t;m}) &\leq  2 \sqrt{T \log\left(\frac 2\delta\right)}\\
        \sum_{t = 1}^T   \bar\ell^{\star}_{\mathtt{01},t}(\hat{w}_{t}) - \ell^{\star}_{\mathtt{01},t}(\hat{w}_{t}) &\leq 2 \sqrt{T \log\left(\frac 2\delta\right)}
    \end{align}
\end{lemma}
\begin{proof}
    Note that
    \begin{equation}
        \ell^{\star}_{\mathtt{01},t}(\hat{w}_{t;m}) - \bar\ell^{\star}_{\mathtt{01},t}(\hat{w}_{t;m}) = \ell^{\star}_{\mathtt{01},t}(\hat{w}_{t;m}) - \ee\left[\ell^{\star}_{\mathtt{01},t}(\hat{w}_{t;m})| \filt_{t-1}\right]
    \end{equation}
    and  similarly for $\hat{w}_t$.  Now note that in the definition of $\hat{w}_t$ and $\hat{w}_{t;m}$, both are measurable with respect to $\filt_{t-1}$ and thus we may apply Azuma's inequality to conclude.
\end{proof}
\begin{lemma}[Smoothed Loss is Lipschitz]\label{lem:smoothnessofloss}
    For any $w, w'$, it holds that
    \begin{equation}
        \abs{\bar\ell^{\star}_{\mathtt{01},t}(w) - \bar\ell^{\star}_{\mathtt{01},t}(w')} \leq \frac{20 d}{\sigma\sqrt{1 - \frac 12 \norm{w - w'}^2}} \cdot \norm{w - w'}
    \end{equation}
\end{lemma}
\begin{proof}
    We use the technique of \Cref{lem:lineardisagreementcover}.  In particular, we note that
    \begin{align}
        \abs{\bar\ell^{\star}_{\mathtt{01},t}(w) - \bar\ell^{\star}_{\mathtt{01},t}(w')} \leq \pp\left(\sign(\inprod{w}{x_t}) \neq \sign(\inprod{w'}{x_t}) | \filt_{t-1}\right) = \pp\left(x_t \in \cD(w,w') | \filt_{t-1}\right)
    \end{align}
    where
    \begin{equation}
        \cD(w, w') = \left\{ x | \inprod{\bar w}{x} = 0 \text{ for some } \bar w = \cos\left(\frac \pi 2 \lambda\right)w + \sin\left(\frac \pi 2 \lambda \right)w' \right\}.
    \end{equation}
    This last equality follows from the proof of \Cref{lem:lineardisagreementcover}.  Suppose that $\inprod{w}{w'} = \cos(\theta)$.  Then once again using the generalized Steiner formula \citep[Theorem 10.20 (ii)]{gray2003tubes} we see that as $\theta \leq \frac \pi2$ the $(d-1)$-dimensional volume of $\cD(w, w')$ is bounded by
    \begin{align}
        \vol_{d-1}(\cD(w, w')) &\leq \int_0^\theta \int_{S^{d-2}} e^t d \vol_{d-2}(\cdot) d t \\
        &\leq \vol_{d-2}(S^{d-2}) (e^{\theta} - 1) \\
        &\leq \vol_{d-2}(S^{d-2}) e^\theta \cdot \theta \\
        &\leq \vol_{d-2}(S^{d-2}) e^{\frac \pi 2} \theta
    \end{align}
    Normalizing by the volume of a $(d-1)$-sphere and observing positive homogeneity, we see that
    \begin{equation}
        \mu(\cD(w, w')) \leq 20 d \arccos(\inprod{w}{w'})    
    \end{equation}
    Applying \Cref{lem:arccosholder} tells us that
    \begin{equation}
        \mu(\cD(w, w')) \leq \frac{20 d}{\sqrt{1 - \frac 12 \norm{w - w'}^2}} \cdot \norm{w - w'}
    \end{equation}
    as desired.
\end{proof}
\begin{lemma}\label{lem:arccosholder}
    Let $w,w'$ be on the unit sphere.  Then
    \begin{equation}
        \arccos(\inprod{w}{w'}) \leq \frac{\norm{w - w'}}{\sqrt{1 - \frac 12 \cdot \norm{w - w'}^2}}
    \end{equation}
\end{lemma}
\begin{proof}
    Note that $\inprod{w}{w'} = 1 - \frac 12 \norm{w - w'}^2$.  Let $a = \frac 12\norm{w - w'}^2$.  Then we see
    \begin{align}
        \arccos(1 - a) &= \int_0^a \frac{d s}{\sqrt{1 - (1 - s)^2}} \\
        &= \int_0^a \frac{d s}{\sqrt{2s} \cdot \sqrt{1 - \frac s2}} \\
        &\leq \frac{1}{\sqrt{1 - \frac a2}} \int_0^a \frac{ds}{\sqrt{2s}} \\
        &= \sqrt{\frac{2a}{1 - \frac a2}}
    \end{align}
    Plugging in $a = \frac 12 \norm{w - w'}^2$ concludes the proof.
\end{proof}
\begin{lemma}[Directional Smoothness Smoothing of Loss functions]\label{lem:directionalsmoothnessofloss}
    For any $w, w'$, it holds that
    \begin{equation}
        \abs{\bar\ell^{\star}_{\mathtt{01},t}(w) - \bar\ell^{\star}_{\mathtt{01},t}(w')} \leq \frac{20 d}{\sigdir \sqrt{1 - \frac 12 \norm{w - w'}^2}} \cdot \norm{w - w'}
    \end{equation}
\end{lemma}
\begin{proof}
    Define
    \begin{equation}
        \cD(w, w') = \left\{ x | \inprod{\bar w}{x} = 0 \text{ for some } \bar w = \bar w(\lambda) = \cos\left(\frac \pi 2 \lambda\right)w + \sin\left(\frac \pi 2 \lambda \right)w' \right\}.
    \end{equation}
    By the same argument as in \Cref{lem:lineardisagreementcover}, it holds that if $\sign(\inprod{w}{x}) \neq \sign(\inprod{w'}{x})$, then $x \in \cD(w, w')$.  Thus we note that
    \begin{equation}
        \abs{\bar\ell^{\star}_{\mathtt{01},t}(w) - \bar\ell^{\star}_{\mathtt{01},t}(w')} \leq \pp\left(\sign(\inprod{w}{x_t}) \neq \sign(\inprod{w'}{x_t}) | \filt_{t-1}\right) = \pp\left(x_t \in \cD(w,w') | \filt_{t-1}\right)
    \end{equation}
    Now fix $\epsilon > 0$ and let $v_0, \dots, v_{1/\epsilon}$ be the points such that
    \begin{equation}
        v_i = \cos\left(\frac \pi 2 i \epsilon\right)w + \sin\left(\frac \pi 2 i \epsilon \right)w'
    \end{equation}
    Noting that our parameterization is a constant speed geodesic on the sphere with respect to the round metric, and applying Lipschitzness of the map, we see that if $\inprod{\bar w(\lambda)}{x} = 0$ for some $\lambda$ then $\abs{\inprod{\bar w(i \epsilon)}{x}} \leq \epsilon \arccos(\inprod{w}{w'})$ for some $i$.  The probability of the latter happening is at most $\frac{2 \epsilon \abs{\arccos(\inprod{w}{w'})}}{\sigdir}$.  Taking a union bound over all values tells us that
    \begin{equation}
        \pp\left(x_t \in \cD(w, w') | \filt_{t-1} \right) \leq \frac{2 \abs{\arccos(\inprod{w}{w'})}}{\sigdir}
    \end{equation}
    Applying \Cref{lem:arccosholder} concludes the proof.
\end{proof}



\begin{lemma}[Wrong Labels Bound] 
    Suppose that for all $a \neq b$, $\norm{\Theta_a^\star - \Theta_b^\star} \geq \Delta$.  Let $T_k$ denote the number of samples observed at the end of the $k^{th}$ epoch.
    \begin{align}
        A_1 &= \frac{500}{\sigma^8 \eta^8}\left(\log\left(\frac{2T_k}{\delta}\right) + \frac d2 \log\left(CB\right) + \log\left(K^4 d^2 T_k\right) \right) \\
        A_2 &= C\frac{B}{\sigma^4 \eta^4} \left(2 + 6 K d^2 \log\left(\frac{KT_k}{\delta}\right)\right) \\
        A_3 &= \frac C{\eta^4 \sigma^4} \left(1 + \epsorac + \nu^2 K d^3 m \log\left(\frac{T_k^2 R^2 B^2 m d K}{\delta}\right) + B^2 R^2 K d^2 (1 + \nu^2) \log^2\left(\frac{KT_k}{\delta}\right)\right)
    \end{align}
    Then with probability at least $1 - \delta$,
    \begin{equation}
        \sum_{t:k(t) = k} \I\{\pi_{k+1}(\hat{g}_{k+1}(x_t)) \ne g^\star(x_t)\} \leq K^2 \max\left(A_1, A_2, \frac{A_3}{\Delta^2}\right)
    \end{equation}
    
\end{lemma}
\begin{proof}
    We begin by decomposing the sum of interest:
    \begin{equation}
        \sum_{t:k(t) = k} \I\{\hat{g}_{k+1}(x_t) \ne g^\star(x_t)\}  = \sum_{a \neq \pi(b)}  \sum_{t:k(t) = k} \I\{\pi \circ \hat{g}_{k+1}(x_t) = a\} \cdot \I\{ g^\star(x_t) = b\} 
    \end{equation}
    where we denote by $\pi$ the following function:
    \begin{equation}
        \pi(a) = \argmin_{1 \leq b \leq K} \norm{\widehat{\Theta}_a - \Theta_b^\star}
    \end{equation}
    and we note that the event that $\yhat_t \neq y_t$ is defined to be the event that $\pi \circ \widehat g_{k+1}(x_t) \neq  g^\star(x_t)$.  To begin, fix some $a$.  Note that by \Cref{thm:parameterrecovery}, for any $b$, if $I_{ab}(\widehat{g}) > \max(A_1, A_2)$ then $\norm{\widehat{\Theta}_a - \Theta_b^\star}^2 \leq \frac{A_3}{\abs{I_{ab}(g)}}$ with probability at least $1 - \delta$.  Thus, if $\abs{I_{ab}(\widehat{g})} \geq \max\left(A_1, A_2, \frac{4 A_3}{\Delta^2}\right)$ then $\norm{\widehat{\Theta}_a - \Theta_b^\star} \leq \frac {\Delta}2$.  Suppose that $\pi(a) \neq b$.  Then
    \begin{align}
        \norm{\widehat{\Theta}_a - \Theta_b^\star} &= \norm{\widehat{\Theta}_a - \Theta_{\pi(a)}^\star + \Theta_{\pi(a)}^\star - \Theta_b^\star} \\
        &\geq \norm{\Theta_{\pi(a)}^\star - \Theta_b^\star} - \norm{\widehat{\Theta}_a - \Theta_{\pi(a)}^\star} \\
        &\geq \Delta - \frac \Delta 2 = \frac{\Delta}{2}
    \end{align}
    This contradicts the conclusion of \Cref{thm:parameterrecovery} on the high probability event if $\abs{I_{ab}(\widehat{g})} \geq \max\left(A_1, A_2, \frac{4 A_3}{\Delta^2}\right)$.  Summing over all possibilities of $a,b$ and adjusting the constant in front of $A_3$ by a factor of 4 concludes the proof.
\end{proof}





    
    In order to define $\algfont{OGDUpdate}$ we need to define the soft margin loss, where for a fixed margin parameter $\gamma$ and fixed $(x_t, y_t)$ with $y_t \in [K]$, we define
    \begin{equation}\label{eq:softmarginmulticlass}
        \widetilde{\ell}_{\gamma, t, \widehat{g}}(\bw) = \max\left( 0, \max_{j \neq \widehat{g}(x_t)}\left(1 - \frac{\inprod{w_{\widehat{g}(x_t)} - w_j}{x_t}}{\gamma}\right) \right)
    \end{equation}
    where $\bw = (w_1, \dots, w_K)$ and $\norm{w_i} = 1$ for all $i$.  We have the following update algorithm:
    
    Before we state our result, we define the functions $\pi_k$ as follows:
    \begin{align}
        \pi_k(i) = \argmin_{1 \leq j \leq K} \norm{\widehat{\Theta}_i^k - \Theta_j^\star}.
    \end{align}
    In words, for each epoch $k$, the ERM oracle has returned a classifier $\widehat{g}_k$ and parameters $\left\{ \widehat{\Theta}_i | 1 \leq i \leq K \right\}$, but there is a lack of identifiability between the classifier $\widehat{g}_k$ and $g^\star$ given by the symmetry of the labels; the function $\pi_k$ resolves this identifiability issue by mapping $i$ to the label $j$ whose associated parameter $\Theta_j^\star$ is most closely approximated by $\widehat{\Theta}_i^k$.  We now provide a theorem that bounds the number of mistakes \Cref{alg:master} makes, where a mistake is made when $\pi$ applied to our predicted class is unequal to $g^\star(\bx_t)$ at time $t$.  We have the following result:

    \begin{theorem}[Online Learning Part]
        Suppose that we are in the above setting.  Then with probability at least $1 - \delta$, it holds that
        \begin{align}
            \sum_{t = 1}^T \I\left[\pi_{k(t)  + 1}\left(\argmax_{1 \leq i \leq K} \inprod{w_i^{k(t)}}{\bx_t}\right) \neq g^\star(\bx_t)\right] &\leq  12 \sqrt{T \log\left(\frac 1\delta\right)} + \frac{20 d m \eta T}{\sigdir \gamma \sqrt{1 - \frac{m^2 \eta^2}{2\gamma^2}}} \\
            &+ \frac{4 K}{\eta} + \frac{\eta T}{\gamma^2} + \left(2 + \frac 2\gamma\right) \frac Tm K^2 \max\left(A_1, A_2, \frac{A_3}{\Delta^2}\right) + \frac{2 K^2 \gamma T}{\sigdir}.
        \end{align}
    \end{theorem}
    \begin{proof}
        In addition to $\widetilde{\ell}_{\gamma,t,\widehat{g}}$ defined above, we introduce the following notation:
        \begin{align}
            i_t^\star = g^\star(\bx_t) && \widehat{i}_t = \argmax_{1 \leq i \leq K} \inprod{w_i^{k(t)}}{\bx_t} && \bar i_t = \widehat{g}_{k(t)+1}(\bx_t)
        \end{align}
        or, in words, $i_t^\star$ is the groundtruth correct label, $\widehat{i}_t$ is the class predicted by the current epoch's linear predictors, and $\bar i_t$ is the class predicted by the ERM trained with the current epoch's data included.  Additionally, let 
        \begin{equation}
            \widetilde{\bw}_t = \Pi_{(S^{d-1})^{\times K}}\left(\widetilde{\bw}^{t-1} - \eta \nabla \widetilde{\ell}_{\gamma, t, \widehat{g}_{k(t)+1}}(\widetilde\bw^{t-1}) \right)
        \end{equation}
        i.e., the predicted weight if we were able to apply gradient descent with the labels predicted by the ERM trained on the current epoch's data.  We also consider the following ``losses'' that we will use in the analysis:
        \begin{align}
            \widehat{\ell}_t(\bw) = \I\left[\widehat{i}_t \neq \bar i_t \right] && \ell_t^\star(\bw) = \I\left[\pi_{k(t)}(\widehat{i}_t) \neq i_t^\star\right] && \bar \ell_t^\star = \ee\left[\ell_t^\star(\bw) | \filt_{t-1}\right]
        \end{align}
        or, in words, $\widehat{\ell}_t$ is the event that our prediction is not equal to that of $\widehat{g}_{k(t) + 1}$, $\ell_t^\star$ is the event that our prediction is not equal to the groundtruth, and $\bar \ell_t^\star$ is the expectation of $\ell_t^\star$ given the history.  We now compute:
        \begin{align}
            \sum_{t = 1}^T \I\left[\pi_{k(t)}(\widehat{i}_t) \neq g^\star(\bx_t)\right]  &= \left(\sum_{t = 1}^T \ell^\star(\bw^k) - \bar \ell(\bw^k)\right) + \left(\sum_{t = 1}^T \bar\ell_t^\star(\bw^k) - \bar \ell_t^\star(\widetilde{\bw}_t)\right) + \sum_{t = 1}^T \bar \ell_t^\star(\widetilde{\bw}_t)
        \end{align}
        Now by \Cref{lem:martingalepart}, the first term is bounded with probability at least $1 - \delta$ by $2 \sqrt{T \log\left(\frac 1 \delta\right)}$.  By \Cref{lem:directionalsmoothnessofloss}, the second term is bounded as
        \begin{align}
            \sum_{t = 1}^T \bar\ell_t^\star(\bw^{k(t)}) - \bar \ell_t^\star(\widetilde{\bw}_t) & \leq \frac{20 d}{\sigdir} \sum_{t = 1}^T \frac{\norm{\widetilde\bw_t - \bw^{k(t)}}}{\sqrt{1 - \frac 12 \norm{\widetilde\bw_t - \bw^{k(t)}}^2 } }
        \end{align}
        Now, note that
        \begin{align}
            \norm{\nabla \widetilde{\ell}_{\gamma, t, \widehat{g}_{k(t) + 1}}(\bw)} \leq \frac{\norm{x_t}}{\gamma} \leq \frac 1\gamma
        \end{align}
        for all $\bw$.  Thus we see that
        \begin{align}
            \norm{\widetilde\bw_t - \bw^{k(t)}} \leq \frac{(t - k(t)) \eta}{\gamma} \leq \frac{m \eta}{\gamma}.
        \end{align}
        Putting this together, we have that with probability at least $1 - 2\delta$,
        \begin{align}
            \sum_{t = 1}^T \bar\ell_t^\star(\bw^{k(t)})  &\leq 2 \sqrt{T \log\left(\frac 1\delta\right)} + \frac{20 d m \eta T}{\sigdir \gamma \sqrt{1 - \frac{m^2 \eta^2}{2\gamma^2}}} + \sum_{t = 1}^T \bar \ell_t^\star(\widetilde{\bw}_t) \\
            &\leq 2 \sqrt{T \log\left(\frac 1\delta\right)} + \frac{20 d m \eta T}{\sigdir \gamma \sqrt{1 - \frac{m^2 \eta^2}{2\gamma^2}}} + \left(\sum_{t = 1}^T \bar \ell_t^\star(\widetilde{\bw}_t) - \ell_t^\star(\widetilde{\bw}_t)\right) + \sum_{t = 1^T} \ell_t^\star(\widetilde{\bw}_t) \\
            &\leq 4\sqrt{T \log\left(\frac 1\delta\right)} + \frac{20 d m \eta T}{\sigdir \gamma \sqrt{1 - \frac{m^2 \eta^2}{2\gamma^2}}} + \sum_{t = 1^T} \ell_t^\star(\widetilde{\bw}_t) 
        \end{align}
        where in the last step we once again applied \Cref{lem:martingalepart}.  Now we note that
        \begin{equation}
            \ell_t^\star(\bw) \leq \widehat{\ell}_t(\bw) + \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right]
        \end{equation}
        Thus, it holds that
        \begin{align}
            \sum_{t = 1}^T \ell_t^\star(\widetilde{\bw}_t) &\leq \sum_{t = 1}^T \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right] + \sum_{t = 1}^T \widetilde{\bw}_t \\
            &\leq \sum_{t = 1}^T \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right] + \sum_{t = 1}^T \widetilde{\ell}_{\gamma, t, \widehat{g}_{k(t)}}(\widetilde{\bw}_t) \\
            &= \sum_{t = 1}^T \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right] + \left(\sup_{\bar \bw} \sum_{t = 1}^T \widetilde{\ell}_{\gamma, t, \widehat{g}_{k(t)}}(\widetilde{\bw}_t) - \widetilde{\ell}_{\gamma, t, \widehat{g}_{k(t)}}(\bar \bw)\right) + \left(\inf_{\bar \bw} \sum_{t = 1}^T \widetilde{\ell}_{\gamma, t, \widehat{g}_{k(t)}}(\bar \bw)\right) 
        \end{align}
        To control the middle term, we see that this expression is just the regret for Online Gradient Descent for losses with gradients bounded in norm by $\frac 1\gamma$ on the $K$-fold product of unit balls, having diameter $2 \sqrt{K}$.  Thus it holds by classical results, such as those found in \citet{hazan2016introduction} that
        \begin{equation}
            \sup_{\bar \bw} \sum_{t = 1}^T \widetilde{\ell}_{\gamma, t, \widehat{g}_{k(t)}}(\widetilde{\bw}_t) - \widetilde{\ell}_{\gamma, t, \widehat{g}_{k(t)}}(\bar \bw) \leq \frac{4 K}{\eta} + \frac{\eta T}{\gamma^2}
        \end{equation}
        We can now apply \Cref{lem:indicatorsoftmargin} to bound the last term, letting $\bw^\star$ be the parameter associated with $g^\star$:
        \begin{align}
            \inf_{\bar \bw} \sum_{t = 1}^T \widetilde{\ell}_{\gamma, t, \widehat{g}_{k(t)}}(\bar \bw) &\leq \inf_{\bar \bw} \sum_{t = 1}^T \I\left[\bx_t \in D_\gamma(\bar \bw)\right] + \left(1 + \frac 2\gamma\right) \widehat{\ell}_t(\bar \bw) \\
            &\leq \inf_{\bar \bw} \sum_{t = 1}^T \I\left[\bx_t \in D_\gamma(\bar \bw)\right] + \left(1 + \frac 2\gamma\right) \left(\sum_{t = 1}^T \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right] + \sum_{t = 1}^T \ell_t^\star(\bar \bw) \right) \\
            &= \left(1 + \frac 2\gamma\right) \sum_{t = 1}^T \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right] + \inf_{\bar \bw} \sum_{t = 1}^T \I\left[\bx_t \in D_\gamma(\bar \bw)\right] + \left(1 + \frac 2\gamma\right) \sum_{t = 1}^T \ell_t^\star(\bar\bw) \\
            &\leq \left(1 + \frac 2\gamma\right) \sum_{t = 1}^T \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right] +  \sum_{t = 1}^T \I\left[\bx_t \in D_\gamma(\bw^\star)\right] + \left(1 + \frac 2\gamma\right) \sum_{t = 1}^T \ell_t^\star(\bw^\star) \\
            &=  \left(1 + \frac 2\gamma\right) \sum_{t = 1}^T \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right] +  \sum_{t = 1}^T \I\left[\bx_t \in D_\gamma(\bw^\star)\right]
        \end{align}
        where we used the fact that $i_t^\star$ is realizable by $\bw^\star$.  Plugging this back in to \eqref{eq:ellstarwtildebound}, we have that
        \begin{align}
            \sum_{t = 1}^T \ell_t^\star(\widetilde{\bw}_t) \leq \frac{4 K}{\eta} + \frac{\eta T}{\gamma^2} + \left(2 + \frac 2\gamma\right) \sum_{t = 1}^T \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right] + \sum_{t = 1}^T \I\left[\bx_t \in D_\gamma(\bw^\star)\right]
        \end{align}
        Now plugging this into \eqref{eq:firstonlineproofineq}, we get that with probability at least $1 - 2 \delta$,
        \begin{align}
            \sum_{t=  1}^T \ell_t^\star(\bw^{k(t)}) \leq 4\sqrt{T \log\left(\frac 1\delta\right)} + \frac{20 d m \eta T}{\sigdir \gamma \sqrt{1 - \frac{m^2 \eta^2}{2\gamma^2}}} + \frac{4 K}{\eta} + \frac{\eta T}{\gamma^2} + \left(2 + \frac 2\gamma\right) \sum_{t = 1}^T \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right] + \sum_{t = 1}^T \I\left[\bx_t \in D_\gamma(\bw^\star)\right]
        \end{align}
        By \Cref{lem:wronglabelsbound}, it holds that with probability at least $1 - \delta$,
        \begin{align}
            \sum_{t = 1}^T \I\left[ \pi_{k(t)}\left(\bar i_t\right) \neq i_t^\star\right] \leq \frac Tm K^2 \max\left(A_1, A_2, \frac{A_3}{\Delta^2}\right)
        \end{align}
        Note that directional smootheness and a union bound tells us that
        \begin{equation}
            \pp\left(\bx_t \in D_\gamma(\bw^\star) | \filt_{t-1}\right) \leq \frac{2 K^2 \gamma}{\sigdir}.
        \end{equation}
        Thus applying \Cref{lem:martingalepart} again, we see that with probability at least $1 - 4 \delta$, it holds that
        \begin{equation}
            \sum_{t=  1}^T \ell_t^\star(\bw^{k(t)}) \leq 6 \sqrt{T \log\left(\frac 1\delta\right)} + \frac{20 d m \eta T}{\sigdir \gamma \sqrt{1 - \frac{m^2 \eta^2}{2\gamma^2}}} + \frac{4 K}{\eta} + \frac{\eta T}{\gamma^2} + \left(2 + \frac 2\gamma\right) \frac Tm K^2 \max\left(A_1, A_2, \frac{A_3}{\Delta^2}\right) + \frac{2 K^2 \gamma T}{\sigdir}
        \end{equation}
        Rescaling $\delta$ concludes the proof.
    \end{proof}

    \begin{lemma}[Bound indicator by soft margin] 
        For any $\gamma, t, \widehat{g}$, it holds that if each component of $\bw$ has unit norm, then
        \begin{equation}
            \widetilde{\ell}_{\gamma,t,\widehat{g}}(\bw) \leq \I\left[\bx_t \in D_\gamma(\bw)\right] + \left(1 + \frac 2\gamma \right)\widehat{\ell}_t(\bw)
        \end{equation}
        where
        \begin{equation}
            D_\gamma(\bw) = \left\{ \bx | \abs{\inprod{w_i - w_j}{\bx_t}} \leq \gamma \text{ for some } 1 \leq i < j \leq K \right\}
        \end{equation}
    \end{lemma}
    \begin{proof}
        We prove this by casework.  Suppose that $\widehat{\ell}_t(\bw) = 0$.  Then it holds that
        \begin{equation}
            \widehat{g}(\bx_t) = \argmax_{1 \leq j \leq K} \inprod{w_j}{\bx_t}
        \end{equation}
        and in particular for all $j \neq \widehat{g}(\bx_t)$, it holds that $\inprod{w_{\widehat{g}(\bx_t) - w_j}}{\bx_t} \geq 0$.  If $\bx_t \not\in D_\gamma(\bw)$ then it holds by construction that
        \begin{equation}
            \max_{j \neq \widehat{g}(\bx_t)} 1 - \frac{\inprod{w_{\widehat{g}(\bx_t)} - w_j}{\bx_t}}{\gamma} \leq 0
        \end{equation}
        and the conclusion clearly holds.  If it holds that
        \begin{equation}
            \max_{j \neq \widehat{g}(\bx_t)} 1 - \frac{\inprod{w_{\widehat{g}(\bx_t)} - w_j}{\bx_t}}{\gamma} > 0
        \end{equation}
        then either there is some $j$ such that $\inprod{w_{\widehat{g}(\bx_t) - w_j}}{\bx_t} < 0$ or there is some $j$ such that $\inprod{w_{\widehat{g}(\bx_t)} - w_j}{\bx_t} < \gamma$ and so $\bx_t \in D_\gamma(\bw)$.  We cannot have the former by the assumption that $\widehat{\ell}_t(\bw) = 0$ so the latter holds and the inequality follows in this case.

        Now suppose that $\widehat{\ell}_t(\bw) = 1$.  Then we see that as $\norm{w_i} = 1$ for all $i$, $\widetilde{\ell}_{\gamma, t, \widehat{g}} \leq \left(1 + \frac 2\gamma\right)$ uniformly and the result holds.
    \end{proof}

